On the Number of Quantifiers as a Complexity Measure

In 1981, Neil Immerman described a two-player game, which he called the "separability game" \cite{Immerman81}, that captures the number of quantifiers needed to describe a property in first-order logic. Immerman's paper laid the groundwork for studying the number of quantifiers needed to express properties in first-order logic, but the game seemed to be too complicated to study, and the arguments of the paper almost exclusively used quantifier rank as a lower bound on the total number of quantifiers. However, last year Fagin, Lenchner, Regan and Vyas rediscovered the games, provided some tools for analyzing them, and showed how to utilize them to characterize the number of quantifiers needed to express linear orders of different sizes. In this paper, we push forward in the study of number of quantifiers as a bona fide complexity measure by establishing several new results. First we carefully distinguish minimum number of quantifiers from the more usual descriptive complexity measures, minimum quantifier rank and minimum number of variables. Then, for each positive integer $k$, we give an explicit example of a property of finite structures (in particular, of finite graphs) that can be expressed with a sentence of quantifier rank $k$, but where the same property needs $2^{\Omega (k^2)}$ quantifiers to be expressed.

==> st-con-and-q-rank.tex <==
% !TEX root = Multi-structural Games ITCS.tex
\begin{proof}
Recall that when we built up the $2\log_2(n)$ expressions in Appendix \ref{app:log_2_method} we started with $s$ and $t$, then added a first point $x_1$ via the expression
\begin{equation}
\exists x_1(E(s,x_1) \land E(x_1,t)).
\end{equation}
Then we used a first universal quantifier to ``pivot'' in the two directions about $x_1$:
\begin{align}
	\exists x_1 \forall x_2 \exists x_3(&x_2 = s \rightarrow E(s,x_3) \land E(x_3, x_1) \land \label{eqn:unnesty} \\
							 (&x_2 = t \rightarrow E(x_1, x_3) \land E(x_3, t)) \notag.
\end{align}
But rather than use the universal quantifier to pivot, we can pivot by using two existential quantifiers nested one level down as follows:
\begin{equation} \label{eqn:1st-nesty}
	\exists x_1(\exists x_2(E(s,x_2) \land E(x_2,x_1)) \land \exists x_2(E(x_1, x_2) \land (E(x_2,t))).
\end{equation}
See Figure \ref{fig:x1-x2}.
\begin{figure} [h]
\centerline{\scalebox{0.60}{\includegraphics{images/x1-x2.png}}}
\caption{The $s$-$t$ connectivity instance described by expression (\ref{eqn:1st-nesty}).}
\label{fig:x1-x2}
\end{figure}

\smallskip

At the next level we can pivot analogously around the two placements of $x_2$, yielding four pivots at the $x_3$ level:
\begin{align}
	\exists x_1(&\exists x_2( \exists x_3(E(s,x_3 \land E(x_3,x_2)) \land \exists x_3(E(x_2,x_3) \land E(x_3, x_1))) \land \label{eqn:2nd-nesty}\\
			     &\exists x_2(\exists x_3(E(x_1, x_3) \land E(x_3, x_2)) \land \exists x_3(E(x_2, x_3) \land E(x_3,t))), \notag
\end{align}
with the associated picture as depicted in Figure \ref{fig:x1-x2-x3}.
\begin{figure} [h]
\centerline{\scalebox{0.60}{\includegraphics{images/x1-x2-x3.png}}}
\caption{The $s$-$t$ connectivity instance described by expression (\ref{eqn:2nd-nesty}).}
\label{fig:x1-x2-x3}
\end{figure}
\medskip

Continuing in this fashion we get expressions of quantifier rank $\log_2(n)$ for instances of STCON($n$).  
\end{proof}

The analogous construction for the expressions that used $3\log_3(n)$ quantifiers in total again nests one level instead of expending a universal quantifier. The expressions look like 
\begin{equation}
\exists x_1 \exists x_2(\exists x_3\exists x_4(...) \land \exists x_3 \exists x_4(...) \land \exists x_3 \exists x_4(...)),
\end{equation}
and so on, yielding expressions of quantifier rank $2\log_3(n)$.



While we observed that $3\log_3(n) < 2 \log_2(n)$ here we have  $\log_2(n) < 2\log_3(n)$ [since $\log_2(n) = \log_2(3) \log_3(n)$ and $\log_2(3) < 2$]. Hence $\log_2(n)+O(1)$ is a tighter upper bound on the quantifier rank needed to express STCON(n). In fact, it is tight up to additive constant due to Theorem~\ref{thm:st-lb}. 

==> t_of_5.tex <==
% !TEX root = Multi-structural Games ITCS.tex

\begin{lemma} \label{lemma:t_of_5_lower}
$t(5) \geq 16$.
\end{lemma}

\begin{proof}
%We shall establish this lower bound by producing an expression of prenex depth $5$ that distinguishes rooted trees of depth $15$ or greater from those of depth less than $15$. The sentence will say, in effect, that there is an element $v$ with a rooted tree of depth $4$ below $v$, and a linear order of size $10$ above $v$. Let us first establish that we can distinguish trees of depth $4$ and above from those of depth less than $4$ via a prenex depth $4$ formula starting with the quantifier sequence $\forall x \exists y \forall z \exists w$, in analogy to the quantifiers used to distinguish linear orders of size $10$ or greater from linear orders of size less than $10$, per the expression for $\Phi_4$ in (\ref{g4}).  The following formula does the trick:
%\begin{align} \label{Tau_4}
%T_4 = \forall x \exists y \forall z \exists w(& \notag \\
%	&x < y \vee(y < x~\land  \\
%	&~~~~~~~~~~~y < z < x \rightarrow (x < w < z \vee  z < w < x)~\land \notag \\
%	&~~~~~~~~~~~z = y \rightarrow y < w < x). \notag
%\end{align}
%It says that for every element $x$ there either is an element $y$ that is greater than $x$, or an element that is three levels less than $x$. It accomplishes the statement that ``there is  an element that is three levels less than $x$'' by virtue of saying, in the $z = y$ equality condition, that there is necessarily an element $w$ between $x$ and $y$. Then the condition $y < z < x$, which is now necessarily satisfied by some $z$, says that there is an additional element $w$ that is either sandwiched between $y$ and four $z$ or $z$ and $x$. 
%
%Thus we see that both $\Phi_4$  (\ref{g4}) and $T_4$ (\ref{Tau_4}) have the same depth-$4$ prenex quantifiers. Let us write, respectively:
%\begin{eqnarray}
% \Psi_4 &=& \forall x \exists y \forall z \exists w~\psi_4 \\
% T_4 &=&  \forall x \exists y \forall z \exists w~\tau_4.
% \end{eqnarray}
% 
% We can thus form a new expression
% \begin{align}
% \exists u  \forall x \exists y \forall z \exists w(& \notag \\
% 	 &x > u \rightarrow \psi_{4,r} ~\land \notag \\
%	 &x < u \rightarrow \tau_{4,r} ~\land \notag \\
%	 &x = u \rightarrow y > u \land w < u).
% \end{align}
% By $psi_{4,r}$ we mean $\psi_4$ \textit{relativized} so that all variables are constrained to be greater than $u$. Analogously, by $\tau_{4,r}$ we mean $\tau_4$ relativized so that all variables are constrained to be \textit{less} than $u$. The lemma follows.

We shall establish this lower bound by producing an expression with $5$ quantifiers that distinguishes rooted trees of depth $16$ or greater from those of depth less than $16$. The sentence will say, in effect, that there is an element $v$ with a rooted tree of depth $5$ below $v$, and a linear order of size $10$ above $v$. Let us first establish that we can distinguish trees of depth $5$ and above from those of depth less than $5$ via a sentence with $4$ quantifiers starting with the quantifier sequence $\forall x \exists y \forall z \exists w$, in analogy to the quantifiers used to distinguish linear orders of size $10$ or greater from linear orders of size less than $10$, per the expression for $\Phi_4$ in (\ref{g4}).  The following formula, derived from $\Phi_{3,\exists}$ (\ref{g3_exists}) does the trick:
\begin{align}
	\Upsilon_4 = \forall w \exists x \forall y \exists z(& \label{Tau_4} \\
		&w < x~\vee (w > x~\land \notag \\
		&~~~~~~~~~~~~~~~~~~~~~~~~(y < x \rightarrow w > z > x~~~\land \notag \\
		&~~~~~~~~~~~~~~~~~~~~~~~~~w > y > x \rightarrow (z \neq y \land w > z > x)~~~\land \notag \\
		&~~~~~~~~~~~~~~~~~~~~~~~~~y = x \rightarrow z < x))) \notag %= \exists x \forall y \exists z \phi_{3,\exists} \notag 
\end{align}
It says that for every element $w$ there either is an element $x$ that is greater than $w$, or a rooted tree of depth at least $4$ less than $w$. 

Thus we see that both $\Phi_4$  (\ref{g4}) and $T_4$ (\ref{Tau_4}) have the same depth-$4$ prenex quantifiers. Let us write, respectively:
\begin{eqnarray}
 \Phi_4 &=& \forall x \exists y \forall z \exists w~\phi_4 \\
 \Upsilon_4 &=&  \forall x \exists y \forall z \exists w~\tau_4.
 \end{eqnarray}
 
 We can thus form a new expression
 \begin{align} \label{t5}
T_5 =  \exists u  \forall x \exists y \forall z \exists w(& \notag \\
 	 &x > u \rightarrow \phi_{4,r} ~\land \notag \\
	 &x < u \rightarrow \tau_{4,r} ~\land \notag \\
	 &x = u \rightarrow y > u \land w < u).
 \end{align}
 By $\phi_{4,r}$ we mean $\phi_4$ \textit{relativized} so that all variables are constrained to be greater than $u$. Analogously, by $\tau_{4,r}$ we mean $\tau_4$ relativized so that all variables are constrained to be \textit{less} than $u$. The lemma follows.
\end{proof}

\begin{lemma} \label{t_of_5_upper}
$t(5) \leq 16$.
\end{lemma}

\begin{proof}
Suppose we are playing a $5$ round game on two rooted trees, $T_x(17)$ and $T_x(16)$, where the two trees are the analogs of those in Figure \ref{fig:19_vs_8_christmas}. As usual, it is not beneficial for Spoiler to play first on $L$, or for that matter, on the shorter main branch of $B$. We consider the possible moves on the main branch of $B$. Suppose first that Spoiler plays on B11, meaning the 11th element along the main (longest) branch of $B$. This move will turn out to be the most challenging 1st round move for Duplicator to parry. In response, Duplicator will make a second copy of $L$ and play L10 on the first copy and L11 on the second copy.  If Spoiler plays next from $B$, say, playing above his 1st round move, Duplicator will play just on the 2nd copy of $L$, where he played L11, mimicking Spoiler's move, and assuring victory since a victory on these boards can only be had on the bottom trees, but we there have a $T_x(6)$ vs. $T_x(5)$, which cannot be won in $3$ moves buy virtue of Lemma \ref{lemma:t_of_3}. Analogously, if Spoiler plays his 2nd round move below his 1st round move on $B$ the Duplicator will just play on the 1st copy of $L$, where he mimics the bottom portion move, again assuring victory since the single board game can only be won on top but a game on linear orders of sizes $10$ and $9$ cannot be won by Spoiler in $3$ rounds (by virtue of $g(3) = 4$).

Thus we may assume that Spoiler plays his 2nd round moves from $L$. In order to win, Spoiler will have to play above the 1st move to get a game that is essentially an l.o.(10) vs. l.o.(9) game on the 1st $L$ board and then play below the 1st move to get a game that is effectively a $T_x(6)$ vs. $T_x(5)$ game on the 2nd $L$ board. However, the $T_x(6)$ vs. $T_x(5)$ game is not winnable by playing first on $L$ since by Lemmas \ref{t_forall_recurrence} and \ref{lemma:t_of_3} we have that $t_\forall(4) = 5$.

Next suppose that Spoiler plays a move that is further down the main branch of $B$ then B11. say $B(K)$ for $K > 11$. Then Duplicator can play $L(K-1)$ on a single board. The only way Spoiler can try to win such a game is by playing all remaining moves above the 1st round moves, but such play would result in a game on two linear orders of size $10$ or greater, which we know to be Duplicator winnable by virtue of $g(4) = 10$. Lastly, suppose Spoiler plays a 1st move that is $B(K)$ for $K < 11$. Duplicator then responds playing $L(K)$ on one board and $L(K-1)$ on a second board, with the effect of forcing Spoiler's 2nd round moves to be on $L$, leading to a Duplicator win, just like in the base case wher Spoiler played a 1st move of B11. The lemma is thus established.
\end{proof}

\begin{cor}
$t(5) = 16$.
\end{cor}

\medskip

Although to this point we have established that $t(r) = 2^{r-1}$, for $1 \leq r \leq 5$, surprisingly, this pattern does \textit{not} continue
and we will see in fact that $t(6) = 28$.

==> tree_calcs.tex <==
% !TEX root = Multi-structural Games ITCS.tex
\begin{lemma} \label{t_lower_of_6}
$t(6) \geq 28$.
\end{lemma}

\begin{proof}
We will produce a sentence that says that there is an element $x$ with a linear order of size $18$ or greater above and a rooted tree of length $9$ or greater below.  

First, from the sentence (\ref{T_4}), with prefix $\exists\forall\exists\exists$, that distinguishes rooted trees of depth $8+$ from those of depth less than $8$, we obtain the analogous sentence, with prefix $\forall\exists\forall\exists\exists$ saying that ``for any $x$ there is either an element above or a tree pf depth $8$ below,'' thus distinguishing rooted trees of depth $9+$ from those of depth $<9$. Call this sentence $\Upsilon_{5,\forall}$.

For the linear order piece of our expression we have to be careful since the sentence distinguishing linear orders of size $g(5)+$ from those of size $<g(5)$ has the prefix $\exists\forall\exists\forall\exists$. However, we can create a sentence with prefix $\forall\exists\forall\exists\exists$ as follows: 
\begin{enumerate}
\item Start with the sentence $\Phi_{3,\forall}$ (\ref{g3_forall}), distinguishing linear orders of size $4+$ from those of size $<4$, with prefix $\forall\exists\exists$.
\item From this sentence, create a sentence saying ``there is an element $x$ with a linear order of size at least $4$ to both the left and right.'' This gives an expression with prefix $\exists\forall\exists\exists$ that distinguishes linear orders of size $9+$ from those of size $<9$.
\item From this last sentence we get a sentence with prefix $\forall\exists\forall\exists\exists$ by saying ``for any $x$ there is a linear order of size at least $9$ to either the left or right.''
\end{enumerate}

The final sentence distinguishes linear orders of size $18+$ from those of size $<18$. Let us call the expression $\Phi_{5,\forall}$. Putting $\Phi_{5,\forall}$ together with the earlier $\Upsilon_{5,\forall}$ now that they have the same quantifiers gives us an expression with prefix  $\exists\forall\exists\forall\exists\exists$ distinguishing rooted trees of depth $28+$ from those of depth less than $28$. The lemma follows.
\end{proof}

The following result about linear orders will come in handy:

\begin{lemma} \label{g_forall_of_5}
$g_\forall(5) = 18$.
\end{lemma}

\begin{proof}
Let us recall the meaning of the statement of this lemma, namely, that if Spoiler is constrained to make his 1st move on $L$, then Duplicator wins a $5$-round multi-structural game if and only if the sizes of both linear orders are at least $18$. We demonstrate this fact by first establishing that Duplicator wins when both linear orders are of size at least $18$, and secondly by establishing that Spoiler wins if one linear order is of size at least $18$ and the other of size less than $18$. That Spoiler wins in the case where both linear orders are of size less than $18$ follows by the same generic argument as that given in the LICS paper.

Let us begin with the base case of l.o.(19) vs. l.o.(18). Clearly the best try for Spoiler is to play L9 (equivalently L10) on his 1st move, to which Duplicator will make a copy of the board and play B9 on one board and B10 on the other, as in Figure \ref{fig:19_vs_18}.
\begin{figure} [h]
\centerline{\scalebox{0.65}{\includegraphics{images/19_vs_18.png}}}
\caption{$5$-round multi-structural game on linear orders of size $19$ and $18$ where Spoiler must play first on $L$ (the little linear order), and plays first on L9. The first move L10 is equivalent.}
\label{fig:19_vs_18}
\end{figure}
It is then clearly best for Spoiler to play his 2nd round moves from $B$, thus trying to win the l.o.(10) vs. l.o.(9) game associated with the top $B$ board. To isolate this board, we will give Spoiler the ability to play atoms, but he will have to play what amounts to a $4$-round l.o.(10) vs l.o.(9) game with atoms, playing his 1st move from $B$. The situation is similar to that we saw earlier.  Clearly the best try for Spoiler is to play B5 (equivalently B6) on his 1st move, to which Duplicator will make a copy of the board and play L5 on one board and L4 on the other, as in Figure \ref{fig:10_vs_9_forall}. 
\begin{figure} [h]
\centerline{\scalebox{0.65}{\includegraphics{images/10_vs_9_forall.png}}}
\caption{$4$-round multi-structural game on linear orders of size $10$ and $9$ where Spoiler must play first on $B$, and plays first on B5. The first move B6 is equivalent.}
\label{fig:10_vs_9_forall}
\end{figure}
Now the game reduces to a $3$-round l.o.(5) vs. l.o.(4) game with atoms where the Spoiler must play first on $L$. But this game is a trivial to analyze win for Duplicator. It follows that the original  l.o.(19) vs. l.o.(18), where Spoiler must play first on $L$ is Duplicator winnable.  The argument with either or both linear orders are of sizes greater than $19$ and $18$ respectively are argued analogously.

Next suppose that we have a $5$-round l.o(18) vs. l.o.(17) game with Spoiler required to play first on $L$. In this case Spoiler will play L9 and the only meaningful moves for Duplicator are to play B9 and B10, as indicated in Figure \ref{fig:18_vs_17}.
\begin{figure} [h]
\centerline{\scalebox{0.65}{\includegraphics{images/18_vs_17.png}}}
\caption{$5$-round multi-structural game on linear orders of size $18$ and $17$ where Spoiler must play first on $L$. He plays L9 when the two consequential Duplicator responses are B9 and B10.}
\label{fig:18_vs_17}
\end{figure}
Spoiler then ignores the the top board and just plays on the bottom board to the left of the first move on $B$, reducing to a $4$-round l.o.(9) vs. l.o.(8) game where Spoiler plays first on $B$. A 2nd round choice of B5 results in a Duplicator response of both the moves L4 or L5 (other moves being inconsequential).  The game then becomes a $3$-round l.o.(4) vs. l.o.(3) game with Spoiler playing first on $L$, which is easily seen to be Spoiler winnable. The lemma follows. [NOTE: the game argument in this last paragraph is a bit redundant since we described the associated $\forall\exists\forall\exists\exists$ formula in the proof of Lemma \ref{t_lower_of_6}.]
\end{proof}

We can now use Lemma \ref{g_forall_of_5} to show that the bound for $t(6)$ established in Lemma \ref{t_lower_of_6} is tight.

\begin{lemma} \label{t_of_6}
$t(6) = 28$.
\end{lemma}

\begin{proof}
We show that Duplicator wins multi-structural games on $T_x(29)$ vs. $T_x(28)$. Extending the argument to larger trees is routine. Suppose Spoiler plays B20 or lower. Then Duplicator plays the usual two moves leaving an identical  top side on one and an identical bottom side on the other, forcing a next move from the Spoiler on the $L$ side. In all cases, there is a linear order of one less above, so at worst a l.o.(19) vs. l.o.(18)., forcing a win on the linear orders since $_\forall(5) = 18$ by the previous lemma. On the other hand, if Spoiler plays B19 or higher, i.e., playing some $B(N)$, then Duplicator plays the analogous move $L(N)$. In the worst case, this leaves a $T_x(10)$ vs. $T_x(9)$ $4$-round game, which is Duplicator winnable by virtue of $t_\forall(5) = 9$ (Lemma \ref{t_forall_recurrence} and Corollary \ref{cor:t_of_4}). Hence the lemma is established.
\end{proof}

\begin{lemma} \label{t_of_7}
$t(7) = 60$.
\end{lemma}

\begin{proof}
We first build the sentence that distinguishes $T_x(60+)$ from  $T_x(<60)$. It will be of the form ``there exists an $x$ with a linear order of size $42$ above and a rooted tree of size $17$ below.  We need to make sure that both subexpressions can be made using the same depth-$6$ prefix quantifiers, beginning with $\forall$.

Firstly, let us consider the expression that there is a linear order (above $x$) of size $42$. That there is such an expression follows from the fact that $g(6) = 42$. But we also know from the proof of Theorem 8.1 in the LICS paper that the values of $g(r)$ for even $r > 4$ are associated with formulas that begin with a $\forall$ quantifier, while for odd $r > 4$, the values of $g(r)$ are associated with formulas with leading $\exists$. Since the formula (\ref{g4}) associated with $g(4)$ has the prefix signature $\forall\exists\forall\exists$ it follows that the formula associated with $g(6)$ has the prefix signature $\forall\exists\forall\exists\forall\exists$.

Next, consider the expression that there is a rooted tree (below $x$) of depth $17$. This expression just comes from tacking the quantifier $\forall$ in front of the expression associated with $t(5) = 16$ given in (\ref{t5}) and hence also has prefix signature $\forall\exists\forall\exists\forall\exists$.

We have thus established a formula of prenex signature $\exists\forall\exists\forall\exists\forall\exists$ distinguishing $T_x(60+)$ from $T_x(<60)$. To complete the proof we must show that Duplicator wins any multi-structural game when the trees are of depth at least $60$. As usual we consider the critical case of $T_x(61)$ vs. $T_x(60)$; the case of larger trees is a simple generalization.  If Spoiler picks an element at or below B44, of general form $B(N)$, then Duplicator plays the two moves $L(N-1)$ and $L(N)$. Such a pair of moves forces Spoiler to play on $L$ and try to win a $6$-round game above the first round moves on the $B(N), L(N-1)$ pair. However, doing so leaves linear orders of sizes at least $2$, with 1st moves constrained to $L$. But $g(6) = 42$ is associated with a formula with a leading universal quantifier, so Duplicator can be assured of being able to win such a game.

On the other hand, if Spoiler picks an element at of above B43, again say of the form $B(N)$, for $N \leq 43$. Then Duplicator picks the associated elements $L(N), L(N-1)$. This time the critical difference is the trees below the first round moves on the $B(N), L(N)$ pair. In this case though, we are left with trees $T_x(18)$ and $T_x(17)$ that must be exploited in a $6$-round game with the constraint that Spoiler next play on $L$. However, Duplicator also wins this game by virtue of the fact that $t_\forall(6) = 17$. The lemma follows.
\end{proof}
